A compactness theorem for Fueter sections

We prove that a sequence of Fueter sections of a bundle of compact hyperkahler manifolds $\mathfrak X$ over a $3$-manifold $M$ with bounded energy converges (after passing to a subsequence) outside a $1$-dimensional closed rectifiable subset $S \subset M$. The non-compactness along $S$ has two sources: (1) Bubbling-off of holomorphic spheres in the fibres of $\mathfrak X$ transverse to a subset $\Gamma \subset S$, whose tangent directions satisfy strong rigidity properties. (2) The formation of non-removable singularities in a set of $\mathcal H^1$-measure zero. Our analysis is based on the ideas and techniques that Lin developed for harmonic maps. These methods also apply to Fueter sections on 4-dimensional manifolds; we discuss the corresponding compactness theorem in an appendix. We hope that the work in this paper will provide a first step towards extending the hyperkahler Floer theory developed by Hohloch-Noetzl-Salamon to general target spaces. Moreover, we expect that this work will find applications in gauge theory in higher dimensions.

==> GammaTangentCones.tex <==
\section{Tangent cones to \texorpdfstring{$(\Gamma,\Theta)$}{(Gamma,Theta)}}
\label{Sec_GammaTangentCones}

We conclude the this article with a slight refinement of the regularity statement of $\Gamma$.

\begin{definition}
  Let $x \in \Gamma$ and let $(r_i)$ be a null-sequence.
  Set
  \begin{equation*}
    \Gamma_i := (\exp\circ s_{r_i})^{-1}\Gamma \qandq
    \Theta_i := (\exp\circ s_{r_i})^*\Theta.
  \end{equation*}
  After passing to a subsequence $\Theta_i\,\cH^1\lfloor\Gamma_i$ weakly converges to a measure of the form $\Theta_*\,\cH^1\lfloor\Gamma_*$, with $\Gamma_* \subset \R^3$ a $1$--dimensional rectifiable set and $\Theta_* \co \R^3 \to [0,\infty)$ an upper semi-continuous map supported on $\Gamma_*$.
  Such a pair $(\Gamma_*,\Theta_*)$ is called a \emph{tangent cone} to $(\Gamma,\Theta)$ at $x$.
\end{definition}

Again, it is important to ask \autoref{Q_UniquenessOfTangentCones}.

Using \autoref{Prop_DeviationFromBeingConical} and \autoref{Prop_DeviationFromBeingBalanced} one can show the following.

\begin{prop}
  If $(\Gamma_*,\Theta_*)$ is a tangent cone to $(\Gamma,\Theta)$, then $\Gamma_*$ is the cone on the finite set $\Gamma_* \cap S^2$:
  \begin{equation*}
    \Gamma_* = \bigcup_{x \in \Gamma_*\cap S^2} [0,\infty)\cdot x.
  \end{equation*}
  $\Theta_*$ is constant on each $(0,\infty)\cdot x$.
  Moreover,
  \begin{equation*}
    \sum_{x \in \Gamma_*\cap S^2} \Theta_*(x) \cdot x = 0.
  \end{equation*}
\end{prop}

This means, in particular, that $\Gamma$ cannot suddenly end at a point and does not contain any kinks.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "FueterCompactness"
%%% End:


==> SingularSetOfU.tex <==
\section{The singular set of \texorpdfstring{$u$}{u}}
\label{Sec_SingularSetOfU}

We now begin to analyse $\sing(u)$.

\begin{prop}
  \label{Prop_SingularMonotonicityFormula}
  The monotonicity formula, i.e., \autoref{Prop_Monotonicity}, holds for $u$.
\end{prop}

Repeating the arguments used earlier immediately establishes the following.

\begin{cor}
  \label{Cor_ThetaUpperSemiContinuous}
  $\Theta_u := \Theta_u^* \co M \to [0,\infty)$ is upper semi-continuous.
\end{cor}

\begin{remark}
  If we had an $\epsilon$--regularity theorem for \emph{singular} Fueter sections, it would follow that $\sing(u) = \Theta_u^{-1}([\epsilon_0,\infty))$ for some $\epsilon_0 > 0$; hence, $\sing(u)$ would be closed.
\end{remark}

\begin{proof}[Proof of \autoref{Prop_SingularMonotonicityFormula}]
  The proof of \autoref{Prop_Monotonicity} uses the fact that $u$ is smooth on all of $M$ only in the application of Stokes' theorem in \eqref{Eq_StokesSection}, i.e., to show that
  \begin{equation*}
      \int_{B_\rho(x)} u^*\rd \Omega = \int_{\del B_\rho(x)} u^*\Omega.
  \end{equation*}

  To see that this still holds in the current situation, fix a cut-off function $\chi$ which is zero on $[0,1]$ and one on $[2,\infty]$, and set
  \begin{equation*}
    \chi_r(x) := \chi(d(x,S)/r).
  \end{equation*}
  By the dominated convergence theorem
  \begin{align*}
    \int_{B_\rho(x)} u^*\rd \Omega
    &= \lim_{r \downarrow 0} \int_{B_\rho(x)} \chi_r u^*\rd \Omega \\
    &=  \int_{\del B_\rho(x)} u^*\Omega - \lim_{r \downarrow 0} \int_{B_\rho(x)} \rd\chi_r \wedge u^* \Omega.
  \end{align*}
  To see that the last term vanishes, recall that $\Omega$ is of type $(0,2)$ and $|\Omega| = O(\ur)$.
  Therefore, $|u^*\Omega| \lesssim r|\nabla u|^2$.
  Since $|\rd \chi_r| \lesssim 1/r$, the integral in the limit is bounded by a constant times
  \begin{equation*}
    \int_{\supp \rd\chi_r} |\nabla u|^2,
  \end{equation*}
  which converges to zero as $r$ goes to zero.
\end{proof}

In the following section we will repeatedly use integration by parts as above.
Each application can be justified in the same way as above.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "FueterCompactness"
%%% End:


==> TangentCones.tex <==
\section{Tangent cones}
\label{Sec_TangentCones}

To further analyse $\sing(u)$ it is customary to study tangent cones.
\begin{definition}
  Let $x \in M$ and let $(r_i)$ be a null-sequence.
  Let $u_{r_i}$ be the rescaling of $u$ centered at $x$;
  see \eqref{Eq_RescaledMap}.
  After passing to a subsequence this converges to a limit $(u_*;\Gamma_*,\Theta_*)$ with $\Gamma_* \subset \R^3$ a $1$--dimensional rectifiable set, $u_* \co \R^3\setminus \Gamma_* \to X$ a Fueter map and $\Theta_* \co \R^3 \to [0,\infty)$ an upper semi-continuous map supported on $\Gamma_*$.
  Such a limit is called a \emph{tangent cone} to $u$ at $x$.
\end{definition}

\begin{remark}
  If $x \notin \sing(u)$, then $u_*$ is the constant map with value $u(x)$ and $\Gamma_* = \emptyset$;
  hence, it is only interesting to consider tangent cones to $x \in \sing(u)$.
\end{remark}

\begin{question}[Uniqueness of tangent cones]
  \label{Q_UniquenessOfTangentCones}
  Is $(u_*;\Gamma_*,\Theta_*)$ independent of the sequence $(r_i)$?
\end{question}

\begin{prop}
  \label{Prop_ConicalTangentCones}
  Every tangent cone $(u_*;\Gamma_*,\Theta_*)$ is conical:
  for all $r > 0$,
  \begin{equation*}
    s_r^*(u_*;\Gamma_*,\Theta_*) = (u_*;\Gamma_*,\Theta_*).
  \end{equation*}
\end{prop}

Combing this with $\cH^1(\sing(u_*)) = 0$ yields the following.

\begin{cor}
  \label{Cor_SingU*0}
  For every tangent cone $(u_*;\Gamma_*,\Theta_*)$, $\sing(u_*) \subset \set{0}$.
\end{cor}

\begin{remark}
  \autoref{Prop_ConicalTangentCones} can be viewed as an affirmative answer to the weaker version of \autoref{Q_UniquenessOfTangentCones}: is $(u_*;\Gamma_*,\Theta_*)$ invariant under rescaling $(r_i)$ to $(r\cdot r_i)$? 
\end{remark}

The proof relies on the following estimate.

\begin{prop}
  \label{Prop_DeviationFromBeingConical}
  Let $U \subset \R^3$ be an open subset and $u \in \Gamma(U, \fX)$ be a possibly singular solution of \eqref{Eq_FueterPerturbed} which arises as a limit of smooth solutions.
  Let $\phi \in C^1_c(\R^3)$ and $R \geq 1$ such that $[1,R]\cdot\supp \phi \subset U$.
  Then
  \begin{equation}
    \label{Eq_DeviationFromBeingConical}
    \begin{split}
      &\left|\int R^{-1}\phi(x/R) |\nabla u|^2(x) \,\rd x - \int \phi(x) |\nabla u|^2(x) \,\rd x\right| \\
      &\quad
      \lesssim \|\phi\|_{C^1} \int_{R\cdot \supp \phi} \Big(\abs{x}\abs{\nabla_r u}\abs{\nabla u} + \abs{\fp \circ u} + |x|^2\delta |\nabla u|^2\Big)\rd x
    \end{split}
  \end{equation}
  with $\delta = |\nabla I| + |F_\fX| + |R|$ as in \eqref{Eq_Delta}.
\end{prop}

\begin{proof}
  Let us first assume that $U$ is flat, $I$ is parallel and $u$ solves \eqref{Eq_FueterMap}.
  The derivative of 
  \begin{equation*}
    f(\rho) := \frac{1}{\rho} \int \phi(x/\rho) |\rd u|^2(x)\, \rd x,
  \end{equation*}
  is
  \begin{align*}
    f'(\rho)
    &=
      -\frac{1}{\rho^2} \int \phi(x/\rho) \cdot \abs{\rd u}^2(x) \,\rd x
      - \frac{1}{\rho^3} \int \abs{x}\del_r\phi(x/\rho) \cdot \abs{\rd u}^2(x) \,\rd x.
  \end{align*}
  Using the identities \eqref{Eq_EnergyFlat} and \eqref{Eq_BoundaryContribution} we obtain
  \begin{equation}
    \label{Eq_II}
    \begin{split}
      -\int \phi(x/\rho)\cdot |\rd u|^2(x)
      &=
        2\int \phi(x/\rho) \sum_{i=1}^3 \rd x_i \wedge u^*\omega_i \\
      &=
        2\int \phi(x/\rho) \,\rd(|x| u^*\omega_{\del_r}) \\
      &=
        -\frac{2}{\rho} \int |x| (\rd \phi)(x/\rho) \wedge u^*\omega_{\del_r} \\
      &=
        -\frac{1}{\rho} \int \Big(|x|(\del_r\phi)(x/\rho)\cdot(2\abs{\del_r u}^2-\abs{\rd u}^2) \\
      &\qquad\qquad\quad
        + 2|x|(\del_1 \phi)(x/\rho)\cdot\omega_{\del_r}(\del_2 u, \del_r u) \\
      &\qquad\qquad\quad
        + 2|x|(\del_2 \phi)(x/\rho)\cdot\omega_{\del_r}(\del_r u, \del_1 u)\Big) \,\rd x.
    \end{split}
  \end{equation}
  (Here we implicitly used the argument from the proof of \autoref{Prop_SingularMonotonicityFormula} to justify the integration by parts.)
  In the expression for $f'(\rho)$ the contributions from $\phi(x\rho)|\rd u|^2(x)$ cancel and thus
  \begin{equation}
    \label{Eq_Drf}
    \abs{f'(\rho)}
    \lesssim
      \rho^{-3}\cdot \|\phi\|_{C^1} \int_{\rho\cdot \supp \phi} \abs{x}\abs{\del_r u}\abs{\rd u} \, \rd x.
  \end{equation}
  This yields the desired estimate by integration.
  
  In general, since $u$ only solves the perturbed Fueter equation, when using \eqref{Eq_Energy} and \eqref{Eq_BoundaryContribution} in the first and the last step of \eqref{Eq_II} we acquire the additional terms of the form
  \begin{equation*}
    \frac{1}{\rho}\int \phi(x/\rho) |\fp\circ u|^2(x) + |x|\del_r \phi(x/\rho) |\fp \circ u|^2(x) \, \rd x
  \end{equation*}
  Moreover, in the second step of \eqref{Eq_II} the additional error term
  \begin{equation*}
    \frac{1}{\rho}\int \phi(x/\rho) O(|x|^2\delta) \abs{\nabla u}^2.
  \end{equation*}
  appears.
\end{proof}

\begin{proof}[Proof of \autoref{Prop_ConicalTangentCones}]
  Applying \autoref{Prop_DeviationFromBeingConical} along $u_{r_i}$ shows that the measure
  \begin{equation*}
    \mu_* = |\rd u_*|^2\,\cH^3 + \Theta_*\,\cH^1\lfloor\Gamma_*
  \end{equation*}
  is conical, since terms on the right-hand side of \eqref{Eq_DeviationFromBeingConical} tend to zero as $r_i \to 0$.
  This implies that $\Gamma_*$ and $\Theta_*$ are conical.
  Moreover, the monotonicity formula shows that $\nabla_ru_* = 0$;
  hence, $u_*$ is conical.
\end{proof}


\subsection{Filtration by tangent cones}
\label{Sec_FiltrationByTangentCones}

Following Simon \cite[Section 3.4]{Simon1996} we define a filtration $S_0 \subset S_1 = \sing(u) $ according to the maximal number of lines a non-trivial tangent cone at $x$ splits off:
\begin{equation*}
  S_k := \set{ x \in \sing(u) : \text{all tangent cones to $u$ at $x$ split off at most $k$ lines} }
\end{equation*}
Here we say that a tangent cones splits of $k$ lines if for some orthogonal splitting $\R^k\oplus \R^{3-k}$ it is the pullback from $\R^{3-k}$.

\begin{remark}
  In our situation a non-trivial tangent cone can split off at most one line.
  This is why the filtration has only two steps. 
\end{remark}

The significance of this filtration is that $\dim S_k \leq k$;
see \cite[Section 3.4, Lemma 1]{Simon1996}.

\begin{prop}
  \label{Prop_TangentConesWithLine}
  If $(u_*;\Gamma_*,\Theta_*)$ is non-trivial and splits of a line $\R \in \R^3$, then $\Gamma_* = \R$, $\Theta_*$ is a positive constant and $u_*$ is constant.
\end{prop}

\begin{proof}
  Certainly we must have $\Gamma_* \subset \R$.
  The Fueter equation and $\R$--translation-invariance forces $u_*|_{\R^2\setminus\set{0}} \to X$ to be holomorphic.
  Since it is also conical, it must be constant.
  Clearly, if $\Gamma_* \neq \emptyset$, then $\Gamma_* = \R$ and $\Theta_*$ is constant.
\end{proof}

\begin{question}
  \label{Q_TangentConesWithLine}
  Can the situation in \autoref{Prop_TangentConesWithLine} occur?
\end{question}

\begin{question}
  \label{Q_GammaNonEmpty}
  Are there tangent cones with $\Gamma_* \neq \emptyset$?
\end{question}

If the answer to \autoref{Q_TangentConesWithLine} is no, then it would follow that $\sing(u)$ is at most $0$--dimensional.

\begin{remark}
  In a closely related situation Chen--Li \cite[Step 1 in the proof of Theorem 4.3]{Chen2000} essentially assert that the answer to \autoref{Q_GammaNonEmpty} is negative.
  However, the author finds himself unable to follow the details of their argument.
\end{remark}


\subsection{Holomorphic sections of the conjugate twistor fibration}
\label{Sec_TwistorFibration}

Tangent maps can be interpreted as follows.
Let $\overline{\Tw}(X) := \fH(X) \times X \iso S^2 \times X$ denote the \emph{conjugate twistor space} of $X$ equipped with the tautological complex structure on $\Tw(X)$, given at $(\xi,x)$ by $(I_{S^2} \oplus -I_\xi)$.
Note the minus in front of $I_\xi$ compared to the usual twistor space defined in Hitchin--Karlhede--Lindström--Roček \cite[Section 3.F]{Hitchin1987}.
The projection $\overline{\Tw}(X) \xrightarrow{\pi} S^2$ is called the \emph{conjugate twistor fibration}.

\begin{prop}
  Let $u\co S^2 \to X$.
  The section $\id\times u \in \Gamma(\overline{\Tw}(X))$ is holomorphic if and only if $x \mapsto u(x/|x|)$ is a Fueter map.
\end{prop}

An example of such a section in case $X$ is the Atiyah--Hitchin manifold was discovered by Chen--Li \cite{Chen2005}.
It is an important open question whether such sections do exist for compact hyperkähler manifolds.


\subsection{Balancing of tangent cones}
\label{Sec_BalancingOfTangentCones}

An interesting property of tangent cones is that they are balanced.

\begin{prop}
  \label{Prop_Balancing}
  If $(u_*;\Gamma_*,\Theta_*)$ is a tangent cone, then
  \begin{equation*}
    \int_{S^2} x\cdot |\rd u_*|^2 = 0
    \qandq
    \sum_{x \in S^2 \cap \Gamma_*} x \cdot \Theta_*(x) = 0.
  \end{equation*}
\end{prop}

\begin{remark}
  The analogous statement for harmonic maps was proved by Lin--Rivière as \cite[Theorem B(iii)]{Lin2002}.
\end{remark}

The proof hinges on the following.

\begin{prop}
  \label{Prop_DeviationFromBeingBalanced}
  If $u \in \Gamma(M, \fX)$ satisfies \eqref{Eq_FueterPerturbed}, then for all $x \in M$ and $v \in \Gamma(B_r(x),TM)$
  \begin{equation*}
    \begin{split}
      &\left|\int_{\del B_r(x)} \<v,\del_r\>\(2|\nabla u|^2 + |\nabla_r u|^2\) - 2 \<\nabla_r u,\nabla_v u\>\right| \\
      &\quad\quad
      \lesssim \int_{\del B_r(x)} r\|\nabla v\|_{L^\infty}|\nabla u|^2 + |\fp \circ u|^2
      + \int_{B_r(x)} \delta|\nabla u|^2 + |\nabla(\fp \circ u)|^2
    \end{split}
  \end{equation*}
  with $\delta = |\nabla I| + |F_\fX| + |R|$ as in \eqref{Eq_Delta}.
\end{prop}

\begin{proof}
  Again, we first asume that $M$ is flat, $\fX = M \times X$, $I$ is parallel and $u$ satisfies \eqref{Eq_FueterMap}.
  We can assume that $v$ is constant, because of the first term on the right-hand side.
  Consider
  \begin{equation*}
    f(x) = \int_{B_r(x)} |\rd u|^2.
  \end{equation*}
  By integration by parts
  \begin{equation*}
    \del_v f(x) = \int_{B_r(x)} \del_v|\rd u|^2 = \int_{\del B_r(x)} \<v,\del_r\> |\rd u|^2.
  \end{equation*}
  On the other hand
  \begin{equation*}
    f(x) = -2\int_{B_r(x)} \sum_{i=1}^3 \rd x^i \wedge u^*\omega_i;
  \end{equation*}
  hence,
  \begin{equation*}
    \del_v f(x)
    = -2\int_{B_r(x)} \sL_v \sum_{i=1}^3 \rd x^i \wedge u^*\omega_i
    = -2\int_{\del B_r(x)} i(v) \sum_{i=1}^3 \rd x^i \wedge u^*\omega_i.
  \end{equation*}
  Choose $(v_1,v_2,v_3) = (\del_r,\del_1,\del_2)$ as in the proof of \autoref{Prop_FlatMonotonicity}.
  Then
  \begin{align*}
    \(i(v) \sum_{i=1}^3 \rd x^i \wedge u^*\omega_i\)(e_1,e_2)
    &= \<I_v \del_1 u, \del_2 u\>
      + \<I_1 \del_2 u - I_2 \del_1 u, \del_v u\> \\
    &=  \<I_v \del_1 u, \del_2 u\>
      - \<\del_r u, \del_v u\>.
  \end{align*}
  A computation shows that
  \begin{equation*}
    \<I_v \del_1 u, \del_2 u\>
    = \<\del_r u,\del_v u\> - \frac12\<v,\del_r\>\abs{\rd u}^2.
  \end{equation*}
  Putting everything together yields
  \begin{equation*}
    \int_{\del B_r} \<v,\del_r\>\(2|\rd u|^2 + |\del_r u|^2\) = 2 \int_{\del B_r} \<\del_r u,\del_v u\>.
  \end{equation*}

  In general, one has to adapt the above argument as in the proof of \autoref{Prop_Monotonicity} and obtains further error terms.
\end{proof}

\begin{proof}[Proof of \autoref{Prop_Balancing}]
  Apply \autoref{Prop_DeviationFromBeingBalanced} along the sequence $u_{r_i}$.
  The terms on the right-hand side converge to zero and, by \autoref{Prop_SingularMonotonicityFormula}, so do the terms involving $\nabla_ru_{r_i}$.
  For all $v \in \Gamma(B_r(x),TM)$
  \begin{equation*}
    \lim_{i\to\infty} \int_{S^2} \<v,\del_r\> |\nabla u_{r_i}|^2
    = \int_{S^2} \<v,x\>\cdot |\rd u_*|^2 + \sum_{x \in S^2 \cap \Gamma_*} \<v,x\> \cdot \Theta_*(x);
  \end{equation*}
  hence,
  \begin{equation*}
    \int_{S^2} x \cdot |\rd u_*|^2 + \sum_{x \in S^2 \cap \Gamma_*} x \cdot \Theta_*(x) = 0.
  \end{equation*}
  The same reasoning applied to $u_*$ directly shows that
  \begin{equation*}
    \int_{S^2} x \cdot |\rd u_*|^2 = 0.
  \end{equation*}
  This concludes the proof.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "FueterCompactness"
%%% End:

